ISAR: A Benchmark for Single- and Few-Shot Object Instance Segmentation and Re-Identification

Most object-level mapping systems in use today make use of an upstream learned object instance segmentation model. If we want to teach them about a new object or segmentation class, we need to build a large dataset and retrain the system. To build spatial AI systems that can quickly be taught about new objects, we need to effectively solve the problem of single-shot object detection, instance segmentation and re-identification. So far there is neither a method fulfilling all of these requirements in unison nor a benchmark that could be used to test such a method. Addressing this, we propose ISAR, a benchmark and baseline method for single- and few-shot object Instance Segmentation And Re-identification, in an effort to accelerate the development of algorithms that can robustly detect, segment, and re-identify objects from a single or a few sparse training examples. We provide a semi-synthetic dataset of video sequences with ground-truth semantic annotations, a standardized evaluation pipeline, and a baseline method. Our benchmark aligns with the emerging research trend of unifying Multi-Object Tracking, Video Object Segmentation, and Re-identification.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> sections/bak/01_introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% Humans have a great capacity of remembering and re-identifying object instances. Given just an RGB image of an object, a human would have little trouble re-identifying that object in any scene context.
% This ability allows being aware of object affordances for object manipulation, efficient mapping of a 3D environment and scene completion among other capabilities.

Object-level scene understanding is fundamental to the development of robust and effective spatial AI systems. The ability for an AI system to accurately perceive objects within a scene is crucial to numerous applications in robotics, augmented reality, navigation, and autonomous vehicles. 

Working towards the goal of general-purpose, spatial AI systems, the research community has become increasingly interested in developing object-level mapping pipelines~\cite{runz2017co, xiao2019dynamic, cui2019sof, volumetric_instance-aware_semantic_mapping, slam++, vmap, Kimera, Fusionpp, kundu2022panoptic, strecke2019fusion, xu2019mid, zhang2020vdo, bescos2021dynaslam, liu2019global} for use in robotics, augmented reality and other spatial AI applications. All of these pipelines assume known object models~\cite{slam++} or an upstream object segmentation pipeline, either to assign a semantic class to static parts of the scene~\cite{volumetric_instance-aware_semantic_mapping, Kimera}, or to deal with dynamic objects separately from the static background mapping and reconstruction~\cite{runz2017co, xiao2019dynamic, cui2019sof, strecke2019fusion, xu2019mid, zhang2020vdo, bescos2021dynaslam, vmap, kundu2022panoptic, liu2019global}. Additionally, systems have been proposed which incrementally build databases of objects and their geometry to help with object manipulation \cite{incremental_object_database, lu2022online}. Such systems also rely on object instance segmentation. 
Crucially, this object-level segmentation is currently produced using learned object segmentation models such as Mask R-CNN~\cite{maskrcnn}, Sharp-Mask~\cite{pinheiro2016learning}, PSPNet~\cite{zhao2017pyramid} or Detic~\cite{detic}. Such learned object segmentation models require classes to be known at training and dataset building time. Fine-tuning them to handle a new class requires annotating thousands of diverse examples and many expensive optimization iterations. To build general-purpose robots and spatial AI systems that can deal with arbitrary objects, one needs to be able to teach them about new objects at run-time. Teaching the spatial AI system and adding new objects to an object tracking and segmentation pipeline should be as easy as selecting the new objects through a user interface. Effectively, this means solving the problem of single- or few-shot object instance segmentation and re-identification. 

So far, the computer vision community has studied the problems of few-shot semantic segmentation, Video Object Segmentation (VOS) and Re-identification (re-ID) individually. While tremendous progress has been made on all of these tasks independently, we can still not teach our spatial AI systems effectively about new objects. Few-shot semantic segmentation systems use dense object segmentation masks, which are expensive to obtain, and they do not make use of the temporal structure in the video data that spatial AI systems inherently operate on. VOS methods perform extremely well, and make full use of video data, but require an initial dense segmentation mask. Further, they do not deal with re-identifying the objects across different \emph{scene contexts}, which inhibits their in-the-wild usability for the previously mentioned tasks. \rev{We define the scene context as the surrounding environment in which an object is recorded, as well as the pose of the objects in the environment}. Thus, existing methods for object instance segmentation and re-identification either do not use the temporal structure of video data, rely on initial dense segmentation masks and/or struggle to re-identify objects across different scenes. Consequently, there is an apparent gap which could be filled by combining few-shot semantic segmentation, VOS and re-ID methods into one approach. 


To address this gap, we propose \textbf{ISAR}, a benchmark and baseline method for single- and few-shot object \textbf{I}nstance \textbf{S}egmentation \textbf{A}nd \textbf{R}e-identification. Our benchmark is designed to accelerate research progress towards robust algorithms that will enable teaching spatial AI systems through a single or a few sparse training examples. We aim to unify few-shot semantic segmentation, Video Object Segmentation (VOS) and Re-identification (re-ID) -- traditionally mostly separately studied research topics. This reflects the emerging trend in recent years towards combining these topics~\cite{mot_lit_review}. As our goal is to build spatial AI systems that can deal with objects in any configuration, including moving objects, we aim to make it hard to rely purely on spatial information as the primary means of object description. Instead, we advocate the development of vision-based object-centric methods, which do not rely on the context in which the object is first perceived. Through this approach, we strive to advance the representations of object instances, \rev{making them more detailed and distinguishable, which in turn may} enable more robust re-identification and object-level mapping of dynamic environments. 
\rev{Our} semi-synthetic benchmark dataset is recorded using the Habitat AI Simulator~\cite{habitat, habitat2} with scenes of Replica~\cite{replica} and the Habitat-Matterport 3D research dataset~\cite{hm3d}, using objects from the YCB dataset~\cite{ycb}.
The dataset and evaluation code are available at \textit{(omitted for anonymity, will be made available after review)}.

To \rev{summarize}, our contributions are the following:
%
\begin{enumerate*}
    \item A semi-synthetic dataset of video sequences with high-quality ground-truth semantic annotations;
    \item A standardized evaluation pipeline to measure the performance of different methods on this task against each other;
    \item A baseline method to segment and re-identify objects
\end{enumerate*}.
